Decay Estimate for some Toy-models related to the Navier-Stokes system

We prove in this paper a decay estimate for scaling invariant local energy solutions for some toy-models related to the incompressible Navier-Stokes system.

==> mymacros.tex <==
\usepackage[utf8]{inputenc}
\usepackage{color}
\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{stmaryrd}
\usepackage{microtype}
\usepackage[T1]{fontenc}
\usepackage{authblk}
\usepackage{stackengine}
%\usepackage{stix}
%\usepackage{esint}
%
\renewcommand\Affilfont{\itshape\large}
%
\usepackage{amscd,verbatim,fancyhdr}
\usepackage{graphicx}
\usepackage{turnstile}
%
\def\tequiv{\ensuremath\sdststile{}{}}
%
%
\usepackage[reqno, namelimits, sumlimits]{amsmath}
%
%
\topmargin 0in
\oddsidemargin 0in
\evensidemargin 0in
\textwidth 6.2in
\textheight 8.5in
\parskip .1in
%
%
\newcommand{\OO}{\Omega}
\newcommand{\ee}{\epsilon}
\newcommand{\al}{\alpha}
\newcommand{\dd}{\delta}
\newcommand{\vtt}{\vartheta}
\newcommand{\vree}{\varepsilon}
\newcommand{\vrr}{\varrho}
\newcommand{\DD}{\Delta}
\newcommand{\lbd}{\lambda}
\newcommand{\Lbd}{\Lambda}
\newcommand{\1}{\mathbb{1}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}

\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}
\DeclareMathOperator*{\dvg}{\mbox{div}}
\DeclareMathOperator*{\curl}{\mbox{curl}}
\DeclareMathOperator*{\essup}{\mbox{ess sup}}

\usepackage{amssymb,amsfonts}
\usepackage{bbold}
\usepackage{multirow}

\usepackage{blindtext}
%
%
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=green,
}
%
%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[theorem]

\newtheorem{lemma}[theorem]{Lemma}

\theoremstyle{remark}
\newtheorem{remark}{Remark}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]

\numberwithin{equation}{section}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand*{\avint}{\mathop{\ooalign{$\int$\cr$-$}}}
\def\Xint#1{\mathchoice
{\XXint\displaystyle\textstyle{#1}}%
{\XXint\textstyle\scriptstyle{#1}}%
{\XXint\scriptstyle\scriptscriptstyle{#1}}%
{\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
\!\int}
\def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$ }
\vcenter{\hbox{$#2#3$ }}\kern-.6\wd0}}

\def\avint{\Xint-}

%%%%%%%%%%%%%%%%%%%%%%%%%%
